Attenuation artifact detection and severity classification in intracoronary OCT using mixed image representations

In intracoronary optical coherence tomography (OCT), blood residues and gas bubbles cause attenuation artifacts that can obscure critical vessel structures. The presence and severity of these artifacts may warrant re-acquisition, prolonging procedure time and increasing use of contrast agent. Accurate detection of these artifacts can guide targeted re-acquisition, reducing the amount of repeated scans needed to achieve diagnostically viable images. However, the highly heterogeneous appearance of these artifacts poses a challenge for the automated detection of the affected image regions. To enable automatic detection of the attenuation artifacts caused by blood residues and gas bubbles based on their severity, we propose a convolutional neural network that performs classification of the attenuation lines (A-lines) into three classes: no artifact, mild artifact and severe artifact. Our model extracts and merges features from OCT images in both Cartesian and polar coordinates, where each column of the image represents an A-line. Our method detects the presence of attenuation artifacts in OCT frames reaching F-scores of 0.77 and 0.94 for mild and severe artifacts, respectively. The inference time over a full OCT scan is approximately 6 seconds. Our experiments show that analysis of images represented in both Cartesian and polar coordinate systems outperforms the analysis in polar coordinates only, suggesting that these representations contain complementary features. This work lays the foundation for automated artifact assessment and image acquisition guidance in intracoronary OCT imaging.

==> images/cms/cms.tex <==
\begin{table}[ht]
    \label{tab:confusion-matrix}
    \centering
    % \caption{Confusion matrices for the ArcNet models at the A-Line level.}
    \vspace{10pt}
    \begin{minipage}{0.48\textwidth}
        \centering
        \caption{Confusion matrix ArcNet Polar}
        \vspace{4pt}
        \begin{tabular}{lccc|c}
            \toprule
            \multirow{2}{*}{} & \multicolumn{3}{c|}{Predicted Class} & \multirow{2}{*}{F-score} \\
            \cmidrule{2-4}
            & BG & Mild & Severe & \\
            \midrule
            \rule[-1ex]{0pt}{3.5ex} BG & 422154 & 4150 & 8840 & 0.97 \\
            \rule[-1ex]{0pt}{3.5ex} Mild & 7212 & 3067 & 4139 & 0.25 \\
            \rule[-1ex]{0pt}{3.5ex} Severe & 9782 & 2958 & 70626 & 0.84 \\
            \bottomrule
        \end{tabular}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \caption{Confusion matrix ArcNet Single}
        \vspace{4pt}
        \begin{tabular}{lccc|c}
            \toprule
            \multirow{2}{*}{} & \multicolumn{3}{c|}{Predicted Class} & \multirow{2}{*}{F-score} \\
            \cmidrule{2-4}
            & BG & Mild & Severe & \\
            \midrule
            \rule[-1ex]{0pt}{3.5ex} BG & 424816 & 2801 & 7527 & 0.97 \\
            \rule[-1ex]{0pt}{3.5ex} Mild & 7380 & 3768 & 3270 & 0.32 \\
            \rule[-1ex]{0pt}{3.5ex} Severe & 6355 & 3230 & 73781 & 0.87 \\
            \bottomrule
        \end{tabular}
    \end{minipage}
    
    \vspace{12pt}

    \begin{minipage}{0.48\textwidth}
    \centering
    \caption{Confusion matrix ArcNet One-Way}
    \vspace{4pt}
        \begin{tabular}{lccc|c}
            \toprule
            \multirow{2}{*}{} & \multicolumn{3}{c|}{Predicted Class} & \multirow{2}{*}{F-score} \\
            \cmidrule{2-4}
            & BG & Mild & Severe & \\
            \midrule
            \rule[-1ex]{0pt}{3.5ex} BG & 421410 & 2910 & 10824 & 0.97 \\
            \rule[-1ex]{0pt}{3.5ex} Mild & 6738 & 3396 & 4284 & 0.31 \\
            \rule[-1ex]{0pt}{3.5ex} Severe & 8160 & 2865 & 72341 & 0.86 \\
            \bottomrule
        \end{tabular}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
    \centering
    \caption{Confusion matrix ArcNet}
    \vspace{4pt}
        \begin{tabular}{lccc|c}
            \toprule
            \multirow{2}{*}{} & \multicolumn{3}{c|}{Predicted Class} & \multirow{2}{*}{F-score} \\
            \cmidrule{2-4}
            & BG & Mild & Severe & \\
            \midrule
            \rule[-1ex]{0pt}{3.5ex} BG & 428059 & 2713 & 4372 & 0.97 \\
            \rule[-1ex]{0pt}{3.5ex} Mild & 7311 & 5095 & 2012 & 0.39 \\
            \rule[-1ex]{0pt}{3.5ex} Severe & 14259 & 3406 & 65701 & 0.85 \\
            \bottomrule
        \end{tabular}
    \end{minipage}
\end{table}

% \begin{figure}[h]
%   \begin{center}
%   \begin{tabular}{c} %% tabular useful for creating an array of images 
%   \includegraphics[width=.25\textwidth]{images/cms/v0_cm.png}
%   \includegraphics[width=.25\textwidth]{images/cms/v1_cm.png}
%   \includegraphics[width=.25\textwidth]{images/cms/v2_cm.png}
%   \includegraphics[width=.25\textwidth]{images/cms/v3_cm.png}
%   \end{tabular}
%   \end{center}
%   \caption[example] 
%   {\label{fig:data}Confusion matrices for the arcnet models.}
% \end{figure} 
